iGibson 2.0: Object-Centric Simulation for Robot Learning of Everyday Household Tasks

Recent research in embodied AI has been boosted by the use of simulation environments to develop and train robot learning approaches. However, the use of simulation has skewed the attention to tasks that only require what robotics simulators can simulate: motion and physical contact. We present iGibson 2.0, an open-source simulation environment that supports the simulation of a more diverse set of household tasks through three key innovations. First, iGibson 2.0 supports object states, including temperature, wetness level, cleanliness level, and toggled and sliced states, necessary to cover a wider range of tasks. Second, iGibson 2.0 implements a set of predicate logic functions that map the simulator states to logic states like Cooked or Soaked. Additionally, given a logic state, iGibson 2.0 can sample valid physical states that satisfy it. This functionality can generate potentially infinite instances of tasks with minimal effort from the users. The sampling mechanism allows our scenes to be more densely populated with small objects in semantically meaningful locations. Third, iGibson 2.0 includes a virtual reality (VR) interface to immerse humans in its scenes to collect demonstrations. As a result, we can collect demonstrations from humans on these new types of tasks, and use them for imitation learning. We evaluate the new capabilities of iGibson 2.0 to enable robot learning of novel tasks, in the hope of demonstrating the potential of this new simulator to support new research in embodied AI. iGibson 2.0 and its new dataset are publicly available at http://svl.stanford.edu/igibson/.

==> 0-preamble.tex <==
% Author: Animesh Garg
% Date : July 2015
% This is a list of common packages needed in a wide range of latex docs for everyday writing.
% ---------------------------------
%floats and figures
% ---------------------------------
\usepackage{graphics}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage[pdftex]{graphicx}
% \usepackage{wrapfig}
\DeclareGraphicsExtensions{.pdf,.png,.jpg}
%\pdfimageresolution200

\usepackage[skip=2pt,font=small]{caption}
\usepackage{subcaption}
%DONT USE BOTH SUBCAPTION AND SUBFIGURE
% \usepackage[center]{subfigure} 
% \usepackage{overpic}
\usepackage[rightcaption]{sidecap}
\usepackage{pbox}

% ---------------------------------
%Math Stuff
% ---------------------------------
\usepackage{mathtools}
\usepackage{amsmath, amssymb, amscd}
\usepackage{ wasysym } %special symbols
\usepackage{amsfonts}
\usepackage{mathptmx} % selects Times Roman as basic font
\usepackage{gensymb} 
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{mdwmath}
% \usepackage{mdwtab}
% \usepackage{eqparbox} %equations

% ---------------------------------
%Symbols
% ---------------------------------
\DeclareMathAlphabet{\mathcal}{OMS}{lmsy}{m}{n}
\DeclareSymbolFont{largesymbols}{OMX}{cmex}{m}{n}
\usepackage{textcomp} %for getting text tilde
%\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
%\DeclareSymbolFontAlphabet{\mathbbold}{bbold}
%\usepackage{dsfont}

% ---------------------------------
%  Algorithms
% ---------------------------------
% http://tex.stackexchange.com/questions/229355/algorithm-algorithmic-algorithmicx-algorithm2e-algpseudocode-confused

\usepackage{algorithm} %float wrapper for algorithms. %dont use with algorithm2e
%should only use one of algorithmic or algorithmicx or algorithm2e
% \usepackage{algorithmic} %least preferred
% \usepackage[ruled,vlined,linesnumbered]{algorithm2e} 
\usepackage{algorithmicx, algpseudocode} %algpseudocode:layout for algorithmicx

% \algtext*{EndFunction}% Remove "end while" text
% \algtext*{EndWhile}% Remove "end while" text
% \algtext*{EndIf}% Remove "end if" text


% ---------------------------------
%Table Stuff
% ---------------------------------
\usepackage{array} %for table entries to be in center of cell
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{booktabs}

% ---------------------------------
%DOCUMENT WIDE
% ---------------------------------
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage[english]{babel} %for hyphenation rules
\usepackage{units}
% \usepackage{siunitx}
\usepackage{bm}
\usepackage{times} % assumes new font selection scheme installed
\usepackage{xspace}
\usepackage{flushend}%balance columns on last page
% \usepackage[yyyymmdd,hhmmss]{datetime}
\usepackage{csquotes}
\usepackage{makeidx}
\usepackage{blindtext}
\let\labelindent\relax
\usepackage{enumitem}

% \usepackage{fixltx2e} %fix latex issue across versions not needed in new latex versions
\usepackage{soul} %text highlighting
\usepackage{subfiles} %individual file compilation--makes it quick 

\usepackage[protrusion=true,expansion=true]{microtype}
\setlength{\emergencystretch}{3em}

\usepackage[yyyymmdd]{datetime}
\renewcommand{\dateseparator}{-}
\date{\protect\formatdate{1}{1}{2001}}

% ---------------------------------
%Bibliography and cross-ref
% ---------------------------------
% The following lines are for IEEE style conflicts with natbibs
% \makeatletter
% \let\NAT@parse\undefined
% \makeatother
% \usepackage[numbers]{natbib}
% \usepackage{cite} %DONT USE NATBIB AND CITE TOGETHER

%hyperlinking
\usepackage{url}
\makeatletter
\g@addto@macro{\UrlBreaks}{\UrlOrds}
\makeatother
\usepackage{color}
\usepackage[usenames,dvipsnames,table]{xcolor}
% \usepackage[pdfborder={0 0 0.5}]{hyperref}
% \usepackage{hyperref}
% \hypersetup{
%     colorlinks=true,
%     linkcolor=black,
%     citecolor=black,
%     filecolor=cyan,
%     urlcolor=black
% }

%=======U S E R  D E F I N E D  M A C R O S=======
% ---------------------------------
% User Comments
% ---------------------------------
\usepackage{marginnote}
% \newcommand{\bibhref}[2]{#2}
\newcommand{\todohl}[1]{{[\hl{#1?}]}}
% \usepackage[disable]{todonotes}
% \usepackage{todonotes}
\usepackage[colorinlistoftodos]{todonotes}
%takes in optional argument
% \newcommand{\tocite}[1]{%
% \textcolor{red}{[cite:\ifthenelse{\equal{#1}{}}{}{#1}?]}
% }

\newcommand{\animesh}[1]{\todo[inline,color=blue!20]{AG: #1}}
\newcommand{\ignore}[1]{}
\newcommand{\etal}{et al.~}

% ---------------------------------
% Label utils
% ---------------------------------

% Usage:
% \figlabel{myfigure} creates \label{fig:myfigure}
% \figref{myfigure} references it
\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{Fig.    \,\ref{fig:#1}}

% Usage:
% \seclabel{mysection} creates \label{sec:mysection}
% \secref{mysection} references it
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section\,\ref{sec:#1}}

\newcommand{\chlabel}[1]{\label{ch:#1}}
\newcommand{\chref}[1]{Chapter\,\ref{ch:#1}}

% Usage:
% \tablabel{mytable} creates \label{tab:mytable}
% \tabref{mytable} references it
\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% space tweaks 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\abovecaptionskip}{0.5mm}
\setlength{\belowcaptionskip}{0mm} 
\setlength{\textfloatsep}{1.5mm}
\setlength{\dbltextfloatsep}{1.5mm}
%\renewcommand{\baselinestretch}{.9945}

\makeatletter
\newenvironment{mcases}[1][l]
 {\let\@ifnextchar\new@ifnextchar
  \left\lbrace
  \def\arraystretch{1.2}%
  \array{@{}l@{\quad}#1@{}}}
 {\endarray\right.}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% symbol definitions for equations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> 1-intro-v1.tex <==
\section{Introduction}
\label{s:intro}


%- Simulation envs in recent years: great but focused only on one type of state: kinematics
%- Why is that a problem? Many tasks require to simulate other types of physics
%- Existing sims with "other" states: AI2thor, but linked to magic actions
%- Our solution
%- 

Recent years we have seen an explosion of simulation environment for embodied AI research~\cite{}. This is the consequence of two converging trends: The first trend is an ``increased supply'' of simulation capabilities. Physics simulators and renderers have been improving over the last years and are currently able to provide highly realistic results (reactions to physical interactions, virtual images). This improvements combine new models of physical processes~\cite{} with higher capacity for computation~\cite{}, and make it possible to simulate realistically agent's interactions with the safety and reproducibility provided by the simulator. The second trend is an ``increased demand'' of data. Dominated by the revolution of deep neural networks, recent robot learning techniques are data hungry: the embodied AI agents learn from a large number of interactions with the environment. 
If these experiences would be collected in the real world, the training process of a robot may take an unreasonable time and wear out the mechanisms.
By using simulation, machine learning approaches applied to embodied AI problems can be trained faster and safer~\cite{}.

Currently, the main goal of the existing simulators in robotics and embodied AI is to compute motion as the result of physical contact interaction between (rigid) bodies, e.g., between the robot and the environment. This is the main physical process involved in robot navigation and several types of manipulation of the environment such as pick-and-place operations~\cite{} or its generalized version, the rearrangement problem~\cite{}. However, it imposes strong limitations on the activities that can be simulated, and thus, studied, solved and benchmarked. Just by looking at the most common everyday activities performed by humans in their homes such as cleaning or cooking, we observe that they require to manipulate other objects' states beyond kinematics (poses), e.g. objects' temperature, level of wetness or dirtiness. These other physical states go beyond the kinematic properties simulated and updated by most simulators for embodied AI research and require to an extended physics simulator.

In this paper, we present a novel simulation environment, \ig, an extension of our previously presented open-source simulator with several advances that make a departure from previous versions and existing simulators. \ig implements a fully functional \textbf{object-centric representation}: simulated worlds in \ig are defined as collections of object instances of known object categories defined by the WordNet taxonomy~\cite{}. \ig assumes that the WordNet categories have been annotated with extended physical states and properties applicable to all object instances of these categories. 

\ig also maintains and updates a set of \textbf{extended physical properties} per object by approximating multiple physical processes. The properties include kinematics (pose, motion, forces) as is common to most robotics simulators, but also object's temperature, wetness level, cleanliness level, toggled state and sliced state.
% \ig maintains and updates temperature for objects in the scenes based on their distance to heat sources and sinks, such as ovens and freezers. It also maintains the level of wetness for objects that can be soaked, and the clean level based on the dust and/or stain elements on their surface. 
These properties reflect directly in the appearance of the objects that changes depending on the extended states.
%temperature/wetness level, and the dust/stain particles can be removed by cleaning the surface. 
%These extended properties enable new household activities to be simulated in \ig.
To complement these states, \ig provides a set of logical predicates that can be applied to single objects or pairs of objects and that define associated \textbf{semantic binary states}. The logical predicates discretize the continuous state updated by the simulator for an object or a pair of objects into a semantically meaningful discrete values. These logical predicates are related to objects' kinematic state (\texttt{onTopOf}, \texttt{insideOf}, \texttt{nextTo}, \texttt{InContactWith}, \texttt{under}, \texttt{verticallyAdjacent}, \texttt{onFloor}) including internal degrees of freedom of articulated objects (\texttt{open}), objects' temperature (\texttt{cooked}, \texttt{burnt}, \texttt{frozen}), level of wetness (\texttt{soaked}), clean level (\texttt{dusted}, \texttt{stained}) and objects' functional properties (\texttt{toggledOn}). 
But \ig implements not only discriminative functions to map the simulated physical state to semantic binary states, but also \textbf{generative functions} to sample valid simulated physical states based on semantic binary descriptions. Simulated worlds can then be described as sets of semantic states that the simulator translates into valid actionable instances. This enables faster prototyping and specification of scenes in \ig as semantically meaningful sets of objects in symbolic state, but also facilitates training of embodied AI agents in multiple instances of tasks with semantically grounded similar initial state.

To facilitate the development of new embodied AI solutions via imitation and to study how humans perform everyday tasks with full observability of their interactions, we include in \ig a \textbf{new virtual reality interface} compatible with the two main commercially available VR systems, Oculus and HTC Vive. All states are logged during execution and can be replayed deterministically. The human demonstrations can be collected in a new version of the iGibson v1.0 set of ecological fully interactive large scenes. \ig includes a rule based mechanism to create \textbf{more densely populated scenes} with semantic distribution for increased realism.

We evaluate \ig by generating multiple novel tasks for embodied AI agents to solve that were not possible before with existing simulation environments. We apply state-of-the-art robot learning algorithms to solve these tasks and analyze how the new \ig capabilities affect training. The training process of these algorithms serve also as testbed for the performance of \ig for rendering and semantic discrete state condition evaluation. 

In summary, \ig presents the following contributions:
\begin{itemize}[
    topsep=0pt,
    noitemsep,
    leftmargin=2pt,
    itemindent=12pt]
\item an object-centric representation where each object in the simulation is an instance of a WordNet category, annotated with additional properties and updatable states, 
\item a set of additional physical properties --temperature, wetness level, and clean level-- maintained and updated by the simulator and that open the door to simulate and study common household activities, 
\item a set of logical predicates applicable to single objects (unary) or pairs of objects (binary) that map the simulated state to a discrete binary equivalent symbolic representation with direct connection to semantics and language,
\item a set of generative functions associated to the logical predicates to sample valid simulated states from given discrete binary symbolic representations,
\item a novel virtual reality interface to study humans in \ig worlds and collect demonstrations,
\item a new rule-based mechanism to populate the iGibson v1.0 large scenes with small objects semantically arranged to increase realism,
\item a set of exemplary new tasks in \ig that could not be simulated before.
\end{itemize}
We hope that \ig will open new avenues of research and development in embodied AI, enabling solutions to interactive household activities that have been understudied before.





==> big_extended_states_fig.tex <==

\begin{figure}
\begin{subfigure}[t!]{0.99\linewidth}
\centering
\includegraphics[width=0.24\linewidth]{example-image-a}
\hfill
\includegraphics[width=0.24\linewidth]{example-image-a}
\hfill
\includegraphics[width=0.24\linewidth]{example-image-a}
\hfill
\includegraphics[width=0.24\linewidth]{example-image-a}
\caption{\textbf{Object temperature:} \textit{(From left to right)} A stove --toggleable heat source by proximity-- is toggled on, and starts to heat a nearby apple; The temperature and appearance of the apple changes due to proximity to the heat source; After the stove is toggled off, the apple changes back to room temperature, keeping the appearance that corresponds to the maximum temperature reached; The temperature system with object that changes temperature, heat sources and sinks, enable visually guided execution of household activities such as cooking.
}
\label{fig:temp}
\end{subfigure}
\begin{subfigure}[t!]{0.99\linewidth}
\centering
\includegraphics[width=0.19\linewidth]{figs/water-off.jpg}
\hfill
\includegraphics[width=0.19\linewidth]{figs/water-on.jpg}
\hfill
\includegraphics[width=0.19\linewidth]{figs/water-collect.jpg}
\hfill
\includegraphics[width=0.19\linewidth]{figs/water-soak.jpg}
\hfill
\includegraphics[width=0.19\linewidth]{example-image-a}
\caption{\textbf{Object wetness level:} \textit{(From left to right)} A sink --toggleable droplet source-- is toggled on, and starts to create droplets; an object that can change its wetness level gets in contact with the droplets and absorbs them, changing its appearance; the wet object can now be used to remove stains; droplets can also be contained in a receptacle and poured on other objects; With the droplets system, iGibson v2.0 provides a simplified liquid simulation for common household activities.
}
\label{fig:wetness}
\end{subfigure}
\begin{subfigure}[t!]{0.99\linewidth}
\centering
\includegraphics[width=0.24\linewidth]{figs/dust1.jpg}
\hfill
\includegraphics[width=0.24\linewidth]{figs/dust2.jpg}
\hfill
\includegraphics[width=0.24\linewidth]{figs/stain1.jpg}
\hfill
\includegraphics[width=0.24\linewidth]{figs/stain2.jpg}
\caption{\textbf{Object cleanliness level:} \textit{(From left to right)} An object is initialized with dust particles that can be cleaned with a cloth; Another object is initialized with stains that require a wet tool (a scrubber) to be removed; Realistic behaviors and motion are required in iGibson v2.0 to change the cleanliness level of the objects.
}
\label{fig:cleanli}
\end{subfigure}
\centering
\begin{subfigure}[t]{0.48\linewidth}%
\includegraphics[width=0.49\linewidth]{example-image-a}%
\hfill%
\includegraphics[width=0.49\linewidth]{example-image-a}%
\caption{\textbf{Object toggling state:} \textit{(From left to right)} An object with updatable toggling state, a TV, that is in off state is toggled on by contacting the \texttt{TogglingLink}; The TV changes to be toggled on and its appear changes accordingly.
}
\label{fig:functionalstate}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.48\linewidth}%
\includegraphics[width=0.49\linewidth]{figs/sliced_before.png}%
\hfill%
\includegraphics[width=0.49\linewidth]{figs/sliced_after.png}%
\caption{\textbf{Object slice state:} \textit{(From left to right)} An object that can change its slice state is initially not sliced. After exerting enough force with the right part of with a slicing tool (the sharp edge of a knife), the object is sliced into two parts. This state change is irreversible. Slicing objects is part of multiple activities in kitchens. 
}
\label{fig:slicedstate}
\end{subfigure}
\caption{Extended object states}
\label{f:all_ext_states}
\vspace{-5em}
\end{figure}

==> sampling_algorithm.tex <==
\begin{algorithm}
\caption{Pose Sampling Algorithm}\label{alg:pose_sampling}
\begin{algorithmic}[1]
\Procedure{SamplePose}{$obj\_a, obj\_b, pred$}\Comment{pred. is one of OnTop, Inside, Dusty, Stained}
\State $required\_space \gets get\_stable\_orientation\_bounding\_box(obj\_a)$
\Statex
\State \textit{// The AABB of object B represents the possible domain of ray sources}
\State $aabb \gets get\_axis\_aligned\_bounding\_box(obj\_b)$
\Statex
\While{$True$}
\State \textit{// Sample a ray origin and direction. This mechanism takes into account the predicate.}
\State \textit{// The origin may be inside the object or above or on the sides etc. as needed.}
\State $origin, direction \gets sample\_ray\_origin(aabb, pred)$
\Statex
\State \textit{// Create a grid of origins around the center origin, matching the size of the base}
\State \textit{// of required\_space, using a random rotation.}
\State $origin\_grid \gets sample\_grid(origin, required\_space)$
\Statex
% \State \textit{// Cast a ray from each origin in the sampled direction.}
% \State \textit{// Results include hit position, normal, object ID.}
\State $ray\_results \gets ray\_cast(origin\_grid, direction)$
\Statex
\If{\textit{there exists a ray that did not hit object $b$}}
\State $continue$
\EndIf
\Statex
\If{\textit{there exists a ray whose hit normal is too different from center ray}}
\State $continue$
\EndIf
\Statex
\State $plane \gets fit\_plane(ray\_results.hit\_points)$
\If{\textit{there exists a hit point too far from the fit plane}}
\State $continue$
\EndIf
\Statex
\State \textit{// Compute a pose for the required space by projecting the hit points onto the plane,}
\State \textit{// computing the displacement and rotation to match the base to the projection,}
\State \textit{// and rotating the full required space cuboid by this amount.}
\State $projected\_points \gets project\_onto\_plane(ray\_results.hit\_points, plane)$
\State $displacement \gets projected\_points.center - required\_space.base.center$
\State $rot \gets least\_sq\_rotation(required\_space.base + displacement, projected\_points)$
\State $sampled\_cuboid \gets rotate(required\_space + displacement, rot)$
\Statex
\If{\textit{$sampled\_cuboid$ is not empty}}
\State $continue$
\EndIf
\Statex
\State \textit{// The sampled pose for the object is the sampled cuboid centroid and its orientation.}
\State \textbf{return} $sampled\_cuboid.center, sampled\_cuboid.orientation$
\EndWhile
\EndProcedure
\end{algorithmic}
\end{algorithm}
